Estimating Principal Components under Adversarial Perturbations

Robustness is a key requirement for widespread deployment of machine learning algorithms, and has received much attention in both statistics and computer science. We study a natural model of robustness for high-dimensional statistical estimation problems that we call the adversarial perturbation model. An adversary can perturb every sample arbitrarily up to a specified magnitude $\delta$ measured in some $\ell_q$ norm, say $\ell_\infty$. Our model is motivated by emerging paradigms such as low precision machine learning and adversarial training. We study the classical problem of estimating the top-$r$ principal subspace of the Gaussian covariance matrix in high dimensions, under the adversarial perturbation model. We design a computationally efficient algorithm that given corrupted data, recovers an estimate of the top-$r$ principal subspace with error that depends on a robustness parameter $\kappa$ that we identify. This parameter corresponds to the $q \to 2$ operator norm of the projector onto the principal subspace, and generalizes well-studied analytic notions of sparsity. Additionally, in the absence of corruptions, our algorithmic guarantees recover existing bounds for problems such as sparse PCA and its higher rank analogs. We also prove that the above dependence on the parameter $\kappa$ is almost optimal asymptotically, not just in a minimax sense, but remarkably for every instance of the problem. This instance-optimal guarantee shows that the $q \to 2$ operator norm of the subspace essentially characterizes the estimation error under adversarial perturbations.

==> algorithms.tex <==


\section{Algorithms}
In this section we describe the convex program that will be used as the main subroutine in our procedure for estimating the top-$r$ principal subspace. For a given data matrix $A \in \R^{n \times m}$ comprising of $m$ samples, we will consider the following convex program that was proposed in \cite{ACCV}. In our setting the program will be run in corrupted data $\tilde{A}$ and the bulk of our analysis will involve showing that the solution output by the program can be used for estimation despite the presence of adversarial perturbations.
The program below takes in as parameters the rank $r$ and the robustness parameter $\kappa$. The intended solution of the following convex program is to find an (orthogonal) projection matrix of rank at most $r$ that satisfies $\norm{\Pi}_{\infty \to 2} \le \kappa$. In fact, the convex program will work for any $q \ge 2$. In what follows we denote by $\ell_{q^*}$ the dual norm of $\ell_q$ i.e., $\tfrac{1}{q^*}+\tfrac{1}{q}=1$; hence for $q=\infty$, the dual norm is $\ell_1$ i.e., $q^*=1$ . For a matrix $M$, we will use $\norm{M}_q$ to denote the entrywise $\ell_q$ norm given by $\big(\sum_{i.j} |M_{ij}|^{q})^{1/q}$. 
%We consider the SDP for the spike model where each column $A_i \sim N(0,I+\theta \cdot \Pi^*)$ for a constant $\theta$ and projection matrix $\Pi$. Given the rank $r$ and $\kappa$, we consider the following SDP:
\begin{align}
& \min \frac{1}{m}\norm{A}_F^2 - \frac{1}{m} \iprod{A A^{\top}, X} \label{sdp:spike}\\
\textit{ subject to } ~& \tr(X)\le r\\
& 0 \preceq X \preceq I\\
& \norm{X}_{q^*} \le r \kappa^{2} \label{sdp:totalnorm}\\
&\norm{X}_{q \to q^*} \le \kappa^2 \label{sdp:robustnorm}
\end{align}

The following lemma shows that one can use the Ellipsoid algorithm to solve in polynomial time the above convex program, while maintaining approximate feasibility of \eqref{sdp:robustnorm} up to a constant factor. 
\begin{lemma}\label{lem:sdpsolving:spike}
For any $q \ge 2$, there exists a constant $c=c(q)\ge 1$ such that the following holds. There is a randomized polynomial time algorithm that given an instance $A \in \R^{n \times m}$ with an optimal solution $X^*$ to the relaxation \eqref{sdp:spike}-\eqref{sdp:robustnorm}, with high probability finds a solution $\widehat{X}$ that is arbitrarily close in objective value compared to $X^*$ such that $\norm{\widehat{X}}_{q \to q^*} \le c \kappa^2$. 
\end{lemma}

We now describe the algorithm that outputs a robust projection matrix $\widehat{\Pi}$ of rank at most $r$. 

\begin{algorithm}[H]
\caption{Finding Robust Low-Rank Projection}

\begin{algorithmic}[1]
\Function{RobustProjection}{data matrix $\tilde{A} \in \R^{m \times n}$, rank $r$, robustness $\kappa$, norm $q$}
\State Solve \eqref{sdp:spike} on $\tilde{A}$ with parameters $\kappa, q, r$ to find a solution $\widehat{X} \succeq 0$ (see Lemma~\ref{lem:sdpsolving:spike}). 
%\For{$i=1,2,\cdots,t$}
%\If{$|P|=1$}
%\State return P
%\EndIf
\State Use SVD on $\widehat{X}$ to find the subspace spanned by the top-$r$ eigenvectors of $\widehat{X}$. Output $\widehat{\Pi}$, the orthogonal projection matrix onto this subspace. 
%\EndFor
\EndFunction \label{algo:projection}
\end{algorithmic}
\end{algorithm}
% We will sometimes omit the parameter $q$ when $q=\infty$. \xnote{30th: do we still need this sentence?}

Our algorithm for estimating the principal components of the covariance matrix in the presence of adversarial perturbations just uses {\sc RobustProjection} as an additional pre-processing step to find a suitable robust subspace for computing the empirical covariance. 
The following algorithm estimates the top-$r$ principal components, and outputs the best rank-$r$ approximation to the the covariance matrix. 


\begin{algorithm}[H]
\caption{Covariance Estimation under Adversarial Perturbations}
\label{algo:covariance}
\begin{algorithmic}[1]
\Function{AdvRobustCovariance}{$4m$ samples $\tilde{A}_1, \dots, \tilde{A}_{4m} \in \R^{n}$, rank $r$, robustness $\kappa$, norm $q$}
\State Split samples into two parts of sizes $m_1, m_2 = 2m$. Let $A^{(1)}, A^{(2)}$ denote these two datasets.   
%\For{$i=1,2,\cdots,t$}
%\If{$|P|=1$}
%\State return P
%\EndIf
\State For each $j \in [m]$, let $A'_j = \tfrac{1}{\sqrt{2}}(\tilde{A}_j - \tilde{A}_{m+j})$ and let $A''_j = \tfrac{1}{\sqrt{2}}(\tilde{A}_{2m+j} - \tilde{A}_{3m+j})$. \label{st:sym}
\State Run \textsc{RobustProjection}$(A', r, \kappa,q)$ to find a $r$-dimensional projection matrix $\widehat{\Pi}$. 
\State Output $\widehat{\Sigma}_r$ to be empirical covariance of $\widehat{\Pi} A''$. 
%\EndFor
\EndFunction
\end{algorithmic}
\end{algorithm}

% We also present the algorithm for mean estimation in the presence of adversarial perturbations.




\iffalse

Let us consider the spiked covariance model, where in addition there are adversarial corruptions to each point. 

\begin{definition}\label{def:spiked_covariance}
The Spiked Covariance model has the following parameters: the signal strength given by parameter $\theta$ and the rank $r$ projection matrix $\Pi^*$ satisfies $\norm{\Pi^*}_{q \to 2} \le \kappa$ for some $\kappa \ge 1$. Then samples $a^{(1)}, a^{(2)}, \dots, a^{(m)}$ are drawn independently from $n$-variate Gaussian $N(0,I+ \theta \Pi^*)$. Finally the input is $\tilde{a}^{(1)}, \dots, \tilde{a}^{(m)}$ where $\norm{a^{(j)}-\tilde{a}^{(j)}}_\infty \le \delta$.    
\end{definition}

In what follows assume that $q=\infty$. We define the model for covariance estimation here.\xnote{I donot know what is a good name here. Feel free to revise.}

\begin{definition}\label{def:general_model}
Given the rank $r$ and robustness $\kappa$, the data points $A_1,\ldots,A_m$ are drawn independently from $n$-variate Gaussian $N(0,\Sigma^*)$ where the covariance matrix $\Sigma^*$ satisfies the following properties:
\begin{enumerate}
    \item Given the eigendecomposition of $\Sigma^*=\sum_{i=1}^n \lambda_i v_i v_i^{\top}$ with $\lambda_1 \ge \lambda_2 \ge \cdots \lambda_n$, let $\Sigma^*=\Sigma_{\bg}+\Sigma_{\sm}$ where $\Sigma_{\bg}$ is constituted by the largest $r$ eigenvectors $\sum_{i=1}^r \lambda_i v_i v_i^{\top}$ and $\Sigma_{\sm}$ is constituted by the rest eigenvectors $\sum_{i=r+1}^n \lambda_i v_i v_i^{\top}$.
    \item The projection matrix $\Pi^*$ of $\Sigma_{\bg}$ satisfies $\|\Pi^*\|_{\infty\rightarrow 2} \le \kappa$.
    %\item $\lambda_{r}-\lambda_{r+1} \ge \theta$.
\end{enumerate}
The goal is to recover the projection matrix $\Pi^*$ of $\Sigma_{\bg}$ given the parameters $r, \kappa$ and a $\delta$-perturbed data matrix $\wt{A} \in \mathbb{R}^{n \times m}$ where the original $i$th row is $A_i$.
\end{definition}
\fi

==> comp_upper.tex <==
\section{Computational Upper Bounds}
\label{sec:comp_upper}
For a given data matrix $\tilde{A} \in \R^{n \times m}$ comprising $m$ samples, we will consider the following convex program that takes in as parameters the rank $r$ and the robustness parameter $\kappa$. The ideal solution (and its intended solution) of the following convex program is the robust projection matrix $\Pi^*$.   
%We consider the SDP for the spike model where each column $A_i \sim N(0,I+\theta \cdot \Pi^*)$ for a constant $\theta$ and projection matrix $\Pi$. Given the rank $r$ and $\kappa$, we consider the following SDP:
\begin{align}
& \min \frac{1}{m}\norm{\tilde{A}}_F^2 - \frac{1}{m} \iprod{\tilde{A} \tilde{A}^{\top}, X} \label{sdp:spike}\\
\textit{ subject to } ~& \tr(X)=r\\
& 0 \preceq X \preceq I\\
& \norm{X}_{1} \le r \kappa^{2} \label{sdp:totalnorm}\\
&\norm{X}_{\infty \to 1} \le \kappa^2 \label{sdp:robustnorm}
\end{align}

\begin{theorem}\label{thm:spike:recovery}[Recovery]
%Let $T_{\infty}(n):=\sqrt{\log n}$ and $T_q(n):=n^{1/q} \cdot \sqrt{q}$ for any $q \in [2,\infty)$. 
For any $\theta, r, \kappa$, and $n$, there is an algorithm that given $m$ samples in $\R^n$ drawn i.i.d. from the spiked covariance model described above whose projection matrix satisfies $\|\Pi^*\|_{\infty \to 2} \le \kappa$, finds with high probability a subspace $\widehat{\Pi}$ %and $\widehat{\Sigma}$ 
% of rank $r$ in polynomial time such that $\|\wh{\Pi}\|_{\infty \to 2} = O(\kappa) $, $$\norm{\widehat{\Pi}^{\perp}\Pi^*}_F^2 \le \frac{c r \kappa^2}{\theta} \Big( \frac{(1+\theta)  \sqrt{\log n}}{\sqrt{m}} + (1+\theta) \delta + \delta^2\Big),
% %\text{ and } \|\wh{\Sigma}-\Sigma^*\|_F^2 \le O\Big((1+\theta_{\max})\frac{r \kappa^2 n^{2/q} \sqrt{\log n}}{\theta_{\min} \sqrt{m}} + \Big)
% $$
$$
\norm{\widehat{\Pi}^{\perp}\Pi^*}_F^2 \le \frac{1}{\theta} \cdot O\Big(\sqrt{(1+\theta)r} \cdot \kappa \delta  + \kappa^2 \delta^2+ \frac{r\kappa^2 (1+\theta) \sqrt{\log n}}{\sqrt{m}}\Big).
$$
\end{theorem}
\xnote{Feel like we assume the error is less than $1$ when rounding $\wt{\Pi}$. Maybe we can omit the $\delta^2 \kappa^2$ term in the error?}

The following lemma shows how well the SDP can be used to recover the ground-truth robust projection in terms of the maximum entry of a certain deviation matrix. % solution correlates with $\Pi^*$.


\begin{lemma} \label{lem:sdprecoveryfromdeviation}
% For the SDP given above on input an instance $\tilde{A}$ that is a $\delta$-perturbation of $A$ (in $\ell_\infty$ norm), where $\E[A A^\top]=I+\theta \Pi^*$. Suppose  
% $$E:= \frac{1}{m} \tilde{A}\tilde{A}^\top - \E[AA^\top] , \text{ then } \norm{\Pi^* - \wh{\Pi}}_F^2 \le  \frac{4r \kappa^2}{\theta} \times  \norm{E}_\infty, \text{ and further } \norm{\wh{\Pi}}_{\infty \to 1} = O(\kappa),  $$
% when $\norm{E}_\infty < \theta/(4 r \kappa^2)$.
Let $\tilde{A}$ be a $\delta$-perturbation of $A$ (in $\ell_\infty$ norm) where $\E[A A^\top]=\Sigma^*$. Let $E:= \frac{1}{m} \tilde{A}\tilde{A}^\top - \E[AA^\top]$ and $\Delta$ denote $\sup_{X \in \mathcal{P}} |\iprod{E,X}|$ for 
\begin{align}
\label{eq:definition-delta}
\mathcal{P} := \{X \in \R^{n \times n}: \tr(X)=r,
0 \preceq X \preceq I,
\norm{X}_{1} \le r \kappa^{2},
\norm{X}_{\infty \to 1} \le \kappa^2\}.
\end{align} We have $\norm{\Pi^* - \wh{\Pi}}_F^2 \le  \frac{4 \Delta}{\theta}, \text{ and further } \norm{\wh{\Pi}}_{\infty \to 2} = O(\kappa)$ when $\Delta \le \frac{r\theta}{8}$. \end{lemma}

%\begin{proofof}{Theorem~\ref{thm:spike:recovery}}
\begin{proof}
Now since the SDP is a relaxation, we have
% \begin{align*}
%     \bigiprod{\tfrac{1}{m} \tilde{A}\tilde{A}^\top, \wh{X}} &\ge     \bigiprod{\tfrac{1}{m} \tilde{A}\tilde{A}^\top, \Pi^*} = \bigiprod{\E[AA^\top], \Pi^*} + \iprod{E, \Pi^*}= r(1+\theta) + \iprod{E,\Pi^*}\\
%     \text{So } \iprod{\E[AA^\top], \wh{X}}+\iprod{E,\wh{X}} &= \iprod{I+\theta \Pi^*, \wh{X}} + \iprod{E,\wh{X}}  \ge r(1+\theta)  - | \iprod{E,\Pi^*}|\\
%     \theta \iprod{\Pi^*, \wh{X}} & \ge  \theta r - \norm{E}_\infty \norm{\wh{X}}_1 - \norm{E}_\infty \norm{\Pi^*}_1 \ge  \theta r - 2 r \kappa^2 \norm{E}_\infty\\
%     \text{Thus } \iprod{\Pi^*, X} & \ge r - 2r\kappa^2 \norm{E}_\infty = r- \eps.
% \end{align*}
\begin{align*}
    \bigiprod{\tfrac{1}{m} \tilde{A}\tilde{A}^\top, \wh{X}} &\ge     \bigiprod{\tfrac{1}{m} \tilde{A}\tilde{A}^\top, \Pi^*} = \bigiprod{\E[AA^\top], \Pi^*} + \iprod{E, \Pi^*}= r(1+\theta) + \iprod{E,\Pi^*}\\
    \text{So } \iprod{\E[AA^\top], \wh{X}}+\iprod{E,\wh{X}} &= \iprod{I+\theta \Pi^*, \wh{X}} + \iprod{E,\wh{X}}  \ge r(1+\theta)  - | \iprod{E,\Pi^*}|\\
    \theta \iprod{\Pi^*, \wh{X}} & \ge  \theta r - |\iprod{E, \wh{X}_1}| - |\iprod{E, \Pi^*}| \ge  \theta r - 2\Delta\\
    \text{Thus } \iprod{\Pi^*, X} & \ge r - 2\frac{\Delta}{\theta} = r- \eps.
\end{align*}
where $\epsilon = 2\Delta/\theta$.
Let $\wh{X}= \sum_{i=1}^n \lambda_i u_i u_i^{\top}$ be the eigendecomposition of $\wh{X}$ with $\lambda_1 \ge \lambda_2 \ge \cdots \ge \lambda_n$ such that $\Pi_{\wh{X}}=\sum_{i=1}^r u_i u_i^{\top}$. Since $\Pi^*$ is a projection matrix, from the above discussion,
\[
\langle \Pi^*, \wh{X} \rangle = \sum_{i=1}^n \lambda_i \|\Pi^* u_i \|^2_2 \ge r-\eps, ~\text{ and }~ \langle \Pi^*, \Pi_{\wh{X}} \rangle = \sum_{i=1}^r \|\Pi^* u_i \|^2_2.
\]
Similarly since $\langle \Pi_{\wh{X}}, \wh{X} \rangle \ge \langle \Pi^*, \wh{X} \rangle \ge r - \eps$, we have
\[
\sum_{i=1}^r \lambda_i=\langle \Pi_{\wh{X}}, \wh{X} \rangle \ge r-\eps.
\]
\noindent At the same time, $\sum_{i=1}^n \lambda_i=\tr(\wh{X})=r$. These imply $\sum_{i=r+1}^n \lambda_i \|\Pi^* u_i \|^2_2 \le \sum_{i=r+1}^n \lambda_i \le \eps$.
So we have 
\[
\langle \Pi^*, \Pi_{\wh{X}} \rangle=\sum_{i=1}^r \|\Pi^* u_i \|^2_2 \ge \sum_{i=1}^r \lambda_i \|\Pi^* u_i \|^2_2 = \sum_{i} \lambda_i \|\Pi^* u_i \|^2_2 - \sum_{i=r+1}^n \lambda_i \|\Pi^* u_i \|^2_2 \ge r-2\eps. 
\]
Finally we note $\lambda_r \ge 1-\eps$ given $\sum_{i=1}^r \lambda_i \ge r-\eps$, which implies $\|\Pi_{\wh{X}}\|_{q \to 2} \le \|\wh{X}\|_{q \to 2}/(1-\eps)=O(\kappa)$. 
%Moreover, we get the required upper bound on $\norm{\Sigma-\Sigma^*}_F^2$ for $\Sigma=\tfrac{1}{m} \Pi_{\wh{X}} AA^T \Pi_{\wh{X}}  - \Pi_{\wh{X}}$ by using Lemma~\ref{lem:recover_sigma}. 
%have $\|\Sigma^*-\Sigma\|_F^2 = (1+\theta_{\max})^2 \cdot O\big( \frac{C(1+\theta_{\max})r \kappa^2 n^{2/q} \sqrt{\log n}}{\theta_{\min} \sqrt{m}} + r^2/m \big)$ for $\Sigma=\Pi \frac{A A^{\top}}{m} \Pi - \Pi$ from Lemma~\ref{lem:recover_sigma}.
This proves the claim. 
\end{proof}

The proof of the Theorem~\ref{thm:spike:recovery} then follows quite directly from the above lemma and the following lemma. 

\begin{lemma}\label{lem:sdp_closeness}
Suppose the data matrix $\tilde{A}$ is drawn from the above model and let $\wh{X}$ be the optimal solution of the SDP. Furthermore, let $\Delta$ be as defined in \eqref{eq:definition-delta}. Then there exists a universal constants $c_1, c_2>0$ such that with probability $0.99$,
% \[
% \Delta \le \frac{r \kappa^2}{\theta}\Big(\frac{ c_1 (1+\theta)\sqrt{\log n}}{\sqrt{m}} + c_2 (1+\theta)\delta + \delta^2 \Big).
% \]
\[
\Delta \le  O\Big( \sqrt{r} \kappa \delta \sqrt{1+\theta} + \kappa^2 \delta^2+ \frac{r \kappa^2 (1+\theta) \sqrt{\log n}}{\sqrt{m}}\Big).
\]
\anote{Changed the first term from $r \kappa \delta$ to $\sqrt{r} \kappa \delta$.}
\end{lemma}

To prove Lemma~\ref{lem:sdp_closeness}, let $E:=\tfrac{1}{m}\tilde{A}\tilde{A}^\top - \E[AA^\top]$. Let $B:=\tilde{A}-A$ represent the adversarial perturbation. %and let $A_{(j)}$ represent the $j$th row of matrix $A$ (i.e., the $m$ dimensional row vector consisting of the $j$th coordinate of all the samples).

\begin{claim}\label{clm:X_to_half_perturbation}
For any $X$ satisfying the SDP constraints in Program~\eqref{sdp:spike}, for any $\delta$-perturbations $\wt{A}$ and $B=\wt{A}-A$, we always have
$\|X^{1/2} B\|_F \le \sqrt{m} \cdot \kappa \delta$ and $\langle B B^{\top}, X \rangle \le m \kappa^2 \delta^2$.
\end{claim}
\begin{proof}
The norm bound $\|X\|_{\infty \to 1} \leq \kappa^2$ along with the fact that for any matrix $M$, $\|M^\top M\|_{\infty \to 1} = \|M\|^2_{\infty \to 2}$, implies that $\|X^{\frac 1 2}\|_{\infty \to 2} \leq \kappa$. Denoting $B_i$ to be the $i$th column of $B$, we get that $\|B_i\|_{\infty} \le \delta$ and
\begin{align*}
    \|X^{\frac 1 2}B\|_F &= \sqrt{\sum_{i=1}^m \|X^{\frac 1 2}B_i\|^2}\\
    &\leq \sqrt{\sum_{i=1}^m \kappa^2 \delta^2} = \sqrt{m} \kappa \delta.
\end{align*}
Next, $\langle B B^{\top}, X \rangle = \|X^{1/2} B\|_F^2 \le m \kappa^2 \delta^2$.
\end{proof}

We will use the following fact extensively in this section.
\begin{fact}\label{fact:eig_trace_ineq}
For any two PSD matrices $A$ and $B$, we always have $\langle A, B \rangle$ is between $\lambda_{\min}(A) \cdot \tr(B)$ and  $\lambda_{\max}(A) \cdot \tr(B)$.
\end{fact}
\begin{proof}
We rewrite $\langle A,B \rangle = \|A^{1/2} B^{1/2}\|_F^2$, which is sandwiched by
$\lambda_{\min}(A^{1/2})^2 \|B^{1/2}\|_F^2 = \lambda_{\min}(A) \cdot \tr(B)$
and $\lambda_{\max}(A^{1/2})^2 \|B^{1/2}\|_F^2 = \lambda_{\max}(A) \cdot \tr(B)$.
\end{proof}

\begin{proofof}{Lemma~\ref{lem:sdp_closeness}}
Using $\E[A]=0$ we have
\begin{align*}
    E&=\frac{1}{m}(A+B)(A+B)^\top - \E[AA^\top] = \frac{1}{m} \Big( BB^\top +B (A-\E[A])^{\top} + (A-\E[A])B^{\top}+  AA^\top \Big) - \E[AA^\top].
\end{align*}
Hence we have that
\begin{align*}
    |\iprod{E,X}| &\leq \frac{1}{m} \iprod{BB^T, X} + \frac{2}{m} \left|\iprod{(A-\E[A])B^T, X}\right| +  \left|\iprod{\frac{1}{m}AA^\top  - \E[AA^\top], X}\right|.
\end{align*}
Next we separately bound each of the terms above. By Claim~\ref{clm:X_to_half_perturbation}, we bound the first term as
\begin{align*}
    \frac{1}{m} \iprod{BB^T, X} = \frac{1}{m} \|X^{1/2} B\|^2_F \leq  \kappa^2 \delta^2. 
\end{align*}

Then we bound the last term as
\begin{align*}
    \iprod{\frac{1}{m}AA^\top  - \E[AA^\top], X} &\leq \|\frac{1}{m}AA^\top  - \E[AA^\top]\|_\infty \|X\|_1\\
    &\leq c_1\frac{r\kappa^2 (1+\theta) \sqrt{\log n}}{\sqrt{m}}.
\end{align*}

To bound the second term we use the fact that for matrices $M_1, M_2, Q_1,$ and $Q_2$, it holds that
$$
\iprod{M_1 M_2, Q_1 Q_2} \leq \|M_1^\top Q_1\|_F \|M_2 Q_2^\top\|_F
$$
to get
\begin{align*}
    \frac{2}{m}\iprod{(A-\E[A])B^T, X} &= \frac{2}{m}\iprod{(A-\E[A])B^T, X^{\frac 1 2}X^{\frac 1 2}}\\
    &\leq \frac{2}{m} \|(A-\E[A])^\top X^{\frac 1 2}\|_F \|X^{\frac 1 2} B \|_F
\end{align*}

By Claim~\ref{clm:X_to_half_perturbation}, $\|X^{\frac 1 2} B \|_F \le \sqrt{m} \kappa \delta$. Note that $
\|(A-\E[A])^\top X^{\frac 1 2}\|^2_F= \langle A A^{\top} ,X\rangle$ given $\E[A]=0$. Then we split it into 
\[
\langle A A^{\top} ,X\rangle = \langle A A^{\top} -E[A A^{\top}], X\rangle + \langle \E[A A^{\top}], X \rangle = O(r\kappa^2 (1+\theta) \sqrt{\log n} \cdot \sqrt{m}) + (1+\theta) r m,
\]
where the first bound comes from the above discussion of the last term and the second bound comes from Fact~\ref{fact:eig_trace_ineq}.

Combining the above bounds we get that the 2nd term is at most
\begin{align*}
    \frac{2}{m}\iprod{(A-\E[A])B^T, X} &\leq \frac{1}{m} \cdot \sqrt{m} \kappa \delta \cdot O\left( r(1+\theta)m + r\kappa^2 (1+\theta) \sqrt{\log n} \cdot \sqrt{m} \right)^{1/2} \\
    & = O(\sqrt{r(1+\theta)}\kappa \delta) + \kappa \delta \cdot O(\frac{(1+\theta) r \kappa^2 \sqrt{\log n}}{\sqrt{m}})^{1/2}\\
    & \le O(\sqrt{r(1+\theta)}\kappa \delta) + O(\kappa^2 \delta^2) + O(\frac{(1+\theta) r \kappa^2 \sqrt{\log n}}{\sqrt{m}})
\end{align*}

Finally we bound the total error as
\begin{align*}
\Delta \le O\Big(\kappa^2 \delta^2 + \sqrt{r(1+\theta)}\kappa \delta + \frac{r\kappa^2 (1+\theta) \sqrt{\log n}}{\sqrt{m}}\Big).
\end{align*}

%we use the fact that $\|X^{\frac 1 2}\|^2_F = Tr(X) = r$. Hence we have
%\begin{align*}
%    \|(A-\E[A])^\top X^{\frac 1 2}\|_F &\leq  \|(A-\E[A])\|_2 \|X^{\frac 1 2}\|_F\\
%    &\leq O( \sqrt{r(1+\theta)} \sqrt{m}).
%\end{align*}

%\xnote{Not sure how to get $\|(A-\E[A])\|_2 \lesssim \sqrt{(1+\theta)m}$. Feel like it is $\Theta(\sqrt{n})$?}

%\xnote{Discussed with Aravindan on Jan 13th: The right bound of $\|(A-\E[A])\|_2$ seems to be $\sqrt{1+\theta} \cdot (\sqrt{n}+\sqrt{m})$. If we wanna avoid the $\sqrt{n}$ dependency, an alternate bound will be $\|(A-\E[A])^\top X^{\frac 1 2}\|^2_F=\langle X, A A^{\top} - \E[A A^{\top}] \rangle \le \|X\|_1 \cdot \|A A^{\top}-\E[A A^{\top}]\|_{\infty}$ like the line after the next one.


%     \norm{E}_\infty &\le \frac{1}{m}\norm{BB^\top}_\infty +  \norm{\frac{1}{m}AA^\top - \E[AA^\top]}_\infty + \frac{2}{m}\norm{B (A-\E[A])^{\top}}_\infty \nonumber\\
%     &\le \norm{B}_\infty \times  \tfrac{1}{m}\max_{j \in [n]} \norm{B_{(j)}}_1  + \frac{c_1 (1+\theta)\sqrt{\log n}}{\sqrt{m}}+ 2\norm{B}_\infty \times  \tfrac{1}{m}\max_{j \in [n]} \norm{(A-\E[A])_{(j)}}_1 \nonumber\\
%     &\le \delta^2 + \frac{c_1 (1+\theta)\sqrt{\log n}}{\sqrt{m}} +  2 (1+\theta) \delta, \label{eq:inftynormbound}
% \end{align}
% with high probability. The last inequality follows since for a $n$-dimensional Gaussian $g$ with variance at most $\sigma^2$ in each direction, $\norm{g}_1 \le O(n \sigma)$ with probability $1-\exp(-\Omega(n))$. 
% This implies the lemma.

\end{proofof}


==> recover_covariance.tex <==
\subsection{Recover covariance matrix}
We show how to recover the covariance matrix thorough the recovery of the projection matrix $\Pi^*$.

\begin{theorem}\label{thm:recover_top_covariance}
Let $A_1,\ldots,A_m$ be data points drawn independently from $N(0,\Sigma^*)$ from Definition~\ref{def:general_model} where the covariance matrix $\Sigma^*=\sum_{i=1}^n \lambda_i v_i v_i^{\top}$ with $\lambda_1 \ge \lambda_2 \ge \cdots \ge \lambda_n$. For convenience, let $\Sigma_{\bg}$ denote the top $r$ eigenspace $\sum_{i=1}^r \lambda_i v_i v_i^{\top}$ and $\Pi^*$ denote its projection. 

Let $\Pi$ be a rank $r$ projection matrix with $\|\Pi-\Pi^*\|_F^2 \le \eps$. Given the perturbation points $\wt{A}_1,\ldots,\wt{A}_m$, we have $\wt{\Sigma}_{\bg}=\Pi (\sum_{i=1}^m \wt{A}_i \wt{A}_i^{\top}) \Pi$ satisfying
\[
\|\wt{\Sigma}_{\bg}-\Sigma_{\bg}\|_F^2 = O(\lambda_1^2 \eps + \lambda_1^2 \cdot r^2/m + \kappa^4 \delta^4 + \lambda_1 \cdot (1+r/m)\cdot \kappa^2 \delta^2) \text{ when } m = \Omega( \lambda_1^2 r^2).
\]
\end{theorem}

\xnote{ I think Pranjal's suggestion is right. Even though the actual alg works for the same batch of data points. To make our life easier, we can use fresh points after obtaining $\Pi$.
}

We state one useful fact about the covariance estimation.
\begin{fact}\label{fact:covariance_est}
Let $\Sigma$ be a covariance matrix of rank $r$ and largest eigenvalue $\lambda_1$. For any $m$, $A_1,\ldots,A_m \sim N(0,\Sigma^*)$ guarantees  that with probability 0.99, $\|\wt{\Sigma}-\Sigma\|_{op} = \lambda_1 \cdot  O(\sqrt{r/m}+r/m)$ for $\wt{\Sigma}=\frac{1}{m} \sum_i A_i A_i^{\top}$. Moreover, it needs $m=O(\lambda_1^2 r^2/\beta)$ to guarantee with prob. 0.99, $\|\wt{\Sigma}-\Sigma\|_{F}^2 \le \beta$ for $\beta<r$.
\end{fact}

In the perturbation-free setting, we use the following lemma to recover $\Sigma_{\bg}$ once we have recovered the robust projection matrix $\Pi^*$ up to good accuracy.

\begin{lemma}\label{lem:recover_sigma}
For any covariance matrix $\Sigma^*=\sum_{i=1}^n \lambda_i v_i v_i^{\top}$ with eigenvalues $\lambda_1 \ge \lambda_2 \ge \cdots \ge \lambda_n$, let $\Sigma_{\bg}=\sum_{i=1}^r \lambda_i v_i v_i^{\top}$ and $\Pi^*$ be the projection matrix of the top $r$ eigenspace. Given any rank $r$ projection $\Pi$ with $\|\Pi^*-\Pi\|_F^2 \le \eps$, for any $m = \Omega( \lambda_1^2 \cdot r^2 )$, we have that with probability 0.99, $\|\wt{\Sigma} - \Sigma_{\bg} \|_F^2 =O( \lambda_1^2 \cdot \eps+\frac{\lambda_1^2 r^2}{m})$ for $\wt{\Sigma}=\Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi$ with $m$ random samples $A_i \sim N(0,\Sigma^*)$.
\end{lemma}
This is extended from Lemma 8.2 in the previous work \cite{ACCV}. For completeness, we provide the proof in Section~\ref{sec:proof_recover_sigma}. Then we finish the proof the Theorem~\ref{thm:recover_top_covariance} by considering the perturbations.

\begin{proofof}{Theorem~\ref{thm:recover_top_covariance}}
We rewrite it using the definitions:
\begin{align*}
    & \|\Pi (\frac{1}{m} \sum_{i=1}^m \wt{A}_i \wt{A}_i^{\top}) \Pi - \Pi^* \Sigma^* \Pi^*\|^2_F\\
    \le & 2 \|\Pi (\frac{1}{m} \sum_{i=1}^m \wt{A}_i \wt{A}_i^{\top}) \Pi - \Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi\|^2_F + 2\|\Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi - \Pi^* \Sigma^* \Pi^*\|^2_F\\
    \le & 2\|\Pi (\frac{1}{m} \sum_{i=1}^m \wt{A}_i \wt{A}_i^{\top}) \Pi - \Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi\|^2_F + O(\lambda_1^2 \eps + \frac{\lambda_1^2 r^2}{m}),
\end{align*}
where we use Lemma~\ref{lem:recover_sigma} in the last step.

For convenience, let $\wt{A}_i=A_i+B_i$ such that $B_i$ is the perturbation on the $i$th data point. We bound the first term 
\begin{align*}
\|\Pi (\frac{1}{m} \sum_{i=1}^m \wt{A}_i \wt{A}_i^{\top}) \Pi - \Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi\|_F & = \|\Pi (\frac{1}{m} \sum_{i=1}^m (A_i + B_i) (A_i + B_i)^{\top} \Pi - \Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi\|_F\\
& \le \|\Pi (\frac{1}{m} \sum_{i=1}^m B_i B_i^{\top}) \Pi\|_F + \| \Pi (\frac{1}{m} \sum_{i=1}^m A_i B_i^{\top}) \Pi\|_F + \| \Pi (\frac{1}{m} \sum_{i=1}^m B_i A_i^{\top}) \Pi\|_F.
\end{align*}
Now we bound each term separately. For the first term, we have
\[\|\Pi (\frac{1}{m} \sum_{i=1}^m B_i B_i^{\top}) \Pi\|_F \le \frac{1}{m} \sum_{i=1}^m \| \Pi B_i B_i^{\top} \Pi \|_F = O(\kappa^2 \delta^2)
\]
because $\Pi B_i$ is a vector of norm at most $O(\kappa \delta)$. For the second term $\| \Pi (\frac{1}{m} \sum_{i=1}^m A_i B_i^{\top}) \Pi\|_F$, we bound it by
\[
\frac{1}{m} \|\Pi A\|_{op} \cdot \|B^{\top} \Pi\|_F \le \frac{1}{m} \cdot \sqrt{\lambda_1 m} \cdot O(1 + \sqrt{r/m})  \cdot \sqrt{m} \kappa \delta = \sqrt{\lambda_1} \cdot O(\sqrt{r/m}+1) \kappa \delta
\]
where we use $\Pi A$ has rank $r$ and covariance expectation $\E[(\Pi A)\cdot (\Pi A)^{\top}]=\Sigma_{\bg}$ to apply Fact~\ref{fact:covariance_est}: with probability 0.99, $\|\Pi \frac{1}{m} A A^{\top} \Pi - \Sigma_{\bg}\|_{op} \le O(\lambda_1 \cdot \sqrt{r/m})$. So $\|\Pi A A^{\top} \Pi\|_{op} \le m \lambda_1 (1 + O(\sqrt{r/m}))$.

From all discussion above, we bound $\|\Pi (\frac{1}{m} \sum_{i=1}^m \wt{A}_i \wt{A}_i^{\top}) \Pi - \Pi^* \Sigma^* \Pi^*\|^2_F$ by
\[
O(\lambda_1^2 \eps + \lambda_1^2 \cdot r^2/m) + O(\kappa^4 \delta^4) + O(\lambda_1 \cdot (1+r/m) \cdot \kappa^2 \delta^2).
\]
\end{proofof}

\subsection{Proof of Lemma~\ref{lem:recover_sigma}}\label{sec:proof_recover_sigma}
We first state the following fact to bound the Frobenius error of the covariance estimation from Theorem~4.7.1 of \cite{Vershynin}.

\begin{fact}\label{fact:recover_sigma}
Given a rank $r$ covariance matrix $\Sigma^*$ with all eigenvalues upper bounded by $\lambda_{\max}$ and projection matrix $\Pi^*$, for any rank $r$ projection $\Pi$ with $\|\Pi^*-\Pi\|_F^2 \le \eps$ and any $\wt{\Sigma}$ (not necessarily rank $r$), we have 
\[
\|\Sigma^*-\Pi \wt{\Sigma} \Pi \|_F^2 \le 8 \lambda^2_{\max} \cdot \eps+2 \| \Pi \Sigma^* \Pi\ - \Pi \wt{\Sigma} \Pi \|_F^2.
\]
\end{fact}
\begin{proof}
At first, we have $\|\Sigma^* - \Pi \wt{\Sigma} \Pi \|_F^2 \le 2 \|\Sigma^* - \Pi \Sigma^* \Pi\|_F^2 + 2 \| \Pi \Sigma^* \Pi\ - \Pi \wt{\Sigma} \Pi \|_F^2$.

Since $\Pi^*$ is the projection matrix of $\Sigma^*$, we have
\[
\|\Sigma^* - \Pi \Sigma^* \Pi \|_F^2 = \|\Pi^* \Sigma^* \Pi^* - \Pi \Sigma^* \Pi \|_F^2 \le 2 ( \|\Pi^* \Sigma^* \Pi^* -\Pi \Sigma^* \Pi^* \|_F^2 + \|\Pi \Sigma^* \Pi^* -\Pi \Sigma^* \Pi \|_F^2 ).
\]
Since $\|AB\|_{F}^2 \le \|A\|^2_{op} \cdot \|B\|_F^2$, we further simplify it as 
\[
2 (\|\Pi^*-\Pi\|^2_F \cdot \|\Sigma^*\|^2_{op} + \|\Sigma^*\|^2_{op} \cdot \|\Pi^*-\Pi\|^2_F) \le 4 \lambda^2_{\max} \cdot \eps.
\]
\end{proof}

We finish the proof of Lemma~\ref{lem:recover_sigma}.

\begin{proofof}{Lemma~\ref{lem:recover_sigma}}
Given $A_i \sim N(0,\Sigma^*)$, we know $\Pi A_i$ is a random vector generated by $N\big( 0, \Pi \Sigma^* \Pi \big)$. So we apply Fact~\ref{fact:covariance_est} to bound $\|\Pi \Sigma \Pi - \Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi \|_{F}^2 \le \delta$. Then we consider $\Sigma_{\bg}$:
\[
\|  \Pi \Sigma \Pi - \Pi \Sigma_{\bg} \Pi\ \|_F = \| \Pi \Sigma_{\sm} \Pi \|_F \le \| (\Pi-\Pi^*) \Sigma_{\sm} \Pi \|_F + \| \Pi^* \Sigma_{\sm} \Pi \|_F.
\]
Since $\Pi^*$ is the projection matrix of $\Sigma_{\bg}$, $\Pi^* \Sigma_{\sm}=\vec{0}$ such that the second term becomes 0. For the first term $\| (\Pi-\Pi^*) \Sigma_{\sm} \Pi \|_F$, we upper bound it by 
\[
\| (\Pi-\Pi^*) \Sigma_{\sm} \Pi \|_F \le \|\Pi-\Pi^*\|_F \cdot \|\Sigma_{\sm}\|_{op} \cdot \|\Pi\|_{op} \le \lambda_1 \cdot \sqrt{\eps}.
\]
From the above discussion, we have 
\[
\|\Pi \Sigma_{\bg} \Pi - \Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi \|_{F}^2 \le 2\|\Pi \Sigma \Pi - \Pi (\frac{1}{m} \sum_{i=1}^m A_i A_i^{\top}) \Pi \|_{F}^2 + 2\| (\Pi-\Pi^*) \Sigma_{\sm} \Pi \|^2_F = O( \delta + \lambda_1^2 \eps ).
\]
The final bound follows from Fact~\ref{fact:recover_sigma} with $\Sigma^*=\Sigma_{\bg}$ there.
\end{proofof}

